Convergent transcriptomic and neuroimaging signature of Autism Spectrum Disorder

Autism Spectrum Disorder (ASD) is a multi-factorial neurodevelopmental disorder, whose causes are still poorly understood. Effective therapies to reduce all the heterogeneous symptoms of the disorder do not exists yet, but behavioural programs started at a very young age may improve the quality of life of the patients. For this reason, many efforts have been dedicated to the research of a reliable biomarker for early diagnosis. Machine learning approaches to distinguish ASDs from healthy controls based on their brain Magnetic Resonance Images (MRIs) have been plagued by the problem of confounders, showing poor classification performance and inconsistency in the biomarker definition. Brain transcriptomics studies, instead, showed some converging results, but being based on data that can be acquired only post-mortem they are not useful for diagnosis. In this work, using an imaging transcriptomics approach, the following results have been obtained. 1) A deep learning based classifier resilient to confounders and able to exploit the temporal dimension of resting state functional MRIs has been developed, reaching an AUC of 0.89 on an independent test set. 2) Five gene network modules involved in ASD have been identified, by analyzing brain transcriptomics data of subjects with ASD and healthy controls. 3) By comparing the brain regions relevant for the classifier obtained in the first step and the brain-wide gene expression profiles of the modules of interest obtained in the second step, it has been proved that the regions that characterize ASD brain at the neuroimaging level are those in which four out of the five gene modules take a significantly high absolute value of expression. These results prove that, despite the heterogeneity of the disorder, it is possible to identify a neuroimaging-based biomarker of ASD, confirmed by transcriptomics.

==> Background/Old_lmm_Net_data_vis.tex <==
\section{LMM background}
\label{sec:bkg_lmm}

This section provides an introduction to linear mixed models (LMMs), explaining what they are and how to properly employ them in an analysis and interpret their results.

LMMs are an extension of simple linear models. As for linear models, the idea is to model the dependency of a certain variable $Y$ on other variables, with the key difference that mixed models allow both fixed effects (FEs) and random effects (REs), as shown in the equation below:

\begin{equation}
    Y = X \beta + Z u + \epsilon
    \label{eq:lmm}
\end{equation}

Where $X$ and $Z$ are the design matrices of fixed and random effects respectively, while $\beta$ and $u$ are their parameter vectors. Finally, $\epsilon$ is a random error term that factors in the fact that the model will never fit the data perfectly.
Obviously, the difference with respect to linear models is the presence of the RE terms $Z$ and $u$.\\
REs are parameters that are allowed to vary throughout the dataset. A typical example can be when the data are acquired in batches, or groups, and there is an expected difference between these groups. In this case, the target variable $Y$ can be thought of as being influenced by the variables in $Z$ in multiple different ways. For example, in the case dealt in this thesis in which $Y$ are GE values, there may be a baseline of GE levels that differs from batch to batch.\\
To model this behaviour, the batch is introduced in the model as a RE, i.e., its influence on $Y$ is allowed to vary across the dataset. 
Random effects are usually of two kinds: random intercepts and random slopes. The case just described is that of a random intercept: a value added to the mixed model formula that varies from batch to batch. Random slopes instead modify the effect that another variable has on $Y$. For example, age may have a stronger effect on GE in some subjects and weaker in others. In this case, the subject variable is introduced as a random slope linked to age.

LMMs have an additional degree of freedom with respect to standard linear models in model selection: once all the covariates that must be included in the analysis have been identified, they must be assigned to either FEs or REs. 
The following criteria, formulated in \cite{fox2015ecological}, can be used to classify a variable as a RE:
\begin{itemize}
    \item the variable is categorical and has a lot of levels;
    \item there are relatively few data on each level, but multiple samples from most of the levels are available
    \item levels are unevenly sampled
\end{itemize}
Variables that do not satisfy these criteria are considered FEs.

Once the model is selected and the analysis run, there is the question of how to interpret the results. The answer differs depending on whether the variable of interest is modeled as a FE or RE. In genetics studies, usually this variable is a case/control one (e.g., ASD/TDC), which is inserted in the model as a FE. For FEs, the LMM analysis returns the magnitude of the effect (i.e., how much being case or control influences GE, the so-called effect size) and a p-value representing its probability of being different from 0, according to the error on the value estimated by the model.
Note that both the size of the effect and its significance (appropriately corrected for the false discovery rate) are relevant, as a large sample may produce small errors and thus high significance at very low p-values, even for very small effects. On the other hand, larger errors on the variable estimates induced by a small sample or the presence of many covariates in the model may attribute low significance even to strong effects.\\
While it is important to take both these figures of merit into account when evaluating FEs, there is not a wide consensus on how to do it, with some studies attributing more importance to significance \cite{zhou2014efficient,jo2013statistical}, others to effect size \cite{sullivan2012using,lee2016alternatives}, and others advocating a more balanced mixed \cite{marot2009moderated,goodman2019proposed}.


\section{Network background}
\label{sec:bkg_network}

This section describes the steps required for constructing a gene co-expression network, following \cite{zhang2005general}. 
Networks are a very intuitive representation of the interactions between their constituents, called nodes. Despite their simplicity, networks and related concepts such as node connectivity, hubs and modules have been demonstrated to be useful for analyzing complex interactions in several biological domains: gene co-expression networks \cite{yang2014gene,tang2018prognostic,saris2009weighted}, protein interactions \cite{kar2009human}, cell interactions \cite{kirouac2009cell} and many others \cite{horvath2011weighted}. 
This discussion focuses on gene co-expression networks, i.e., networks in which genes are linked to each other based on the correlation between their expression values across several samples or subjects, but the considerations made are valid for any kind of network.\\
The construction of a network (graphically summarized in fig. \ref{fig:network-construction}) articulates in three steps:
\begin{enumerate}
    \item Definition of a similarity matrix, $s_{i,j}$, that quantifies the similarity between pairs of genes, usually through correlation.
    \item Definition of a family of adjacency functions $f_p(s_{i,j})$, used to transform the similarity matrix by suppressing small correlations and enhancing large ones.
    \item Selection of the best adjacency function $f^*$ and construction of the adjacency matrix $a_{i,j}=f^*(s_{i,j})$.
\end{enumerate}

At the end of the last step, the network is fully constructed, and it can be visualized and operated on. It can then be further analyzed to extract meaningful information. A common way to proceed is the identification of network modules, i.e., groups of genes that are similar to each other. This is done in two steps:

\begin{enumerate}
    \item Definition of a measure of gene dissimilarity based on the adjacency matrix, used to calculate which genes are more similar to each other with respect to the rest of the network. Note that this is a different concept from the similarity matrix, because the latter is defined pairwise without considering the rest of the genes in the network.
    \item Identification of network modules using a clustering algorithm on the dissimilarity matrix.
\end{enumerate}

The following sections provide an in-depth description of all the steps reported above.

\begin{figure}
    \centering
    \includegraphics[width=0.99 \textwidth]{Figures/Fig_Bkg_Genetics/network-construction.png}
    \caption{Graphical representation of the steps required for constructing a signed gene co-expression network.}
    \label{fig:network-construction}
\end{figure}

\subsection{Similarity matrix}
The similarity matrix is a matrix weighing the pairwise similarity of genes with a number between 0 and 1, where 1 indicates perfect similarity.
It is commonly defined starting from the pearson correlation between pairs of genes across the available samples: $\rho(G_i,G_j)$.
The similarity matrix is then derived applying a transformation on the correlation values, depending on whether one wants to preserve the sign of the correlation or not, building a \textit{signed} or \textit{unsigned} network respectively.\\
For an \textit{unsigned} network, the absolute value of the correlation is taken: $s_{i,j}=|\rho(G_i,G_j)|$, while for a \textit{signed} network, the correlation is transformed in the following way: $s_{i,j}=(1+\rho(G_i,G_j))/2$. If the first (second) transformation is applied, genes perfectly anti-correlated to each other will have a transformed similarity value of 1 (0).
Note that obviously $s_{i,i}=1$, since every node is perfectly similar to itself, however, for the purpose of calculating all the network concepts described in the following section, it is assumed by convention that the diagonal elements of the similarity matrix are set to 0, as it simplifies many formulas.

\subsection{Definition of the family of adjacency functions}
After constructing the similarity matrix and appropriately transforming it, the adjacency matrix must be derived from it. In order to do this, several adjacency functions are tested and the best one is selected. Usually, functions belonging to the same family all have a common base form, with one or two parameters that distinguish them from each other. Common examples are:
\begin{itemize}
    \item Powers: $f_p(s_{i,j})=s^p_{i,j}$.
    \item Sigmoids: $f_{a,b}(s_{i,j}=\frac{1}{1+e^{-a(s_{i,j}-b)}}$
    \item Hard thresholds: $ f_{t}(s_{i,j}) = \begin{cases}
      0 &  \text{if }x < t \\
      1 &  \text{if }x \geq t
    \end{cases}\, $
\end{itemize}
The first two families of functions can be described as soft thresholds and generate weighted networks, i.e., networks in which the connection between two genes is represented by a weight in the interval $[0,1]$, with 1 being the strongest connection and 0 being the weakest one. Many other families of soft thresholds have been proposed in literature, but they all behave very similarly to each other \cite{zhang2005general}. The key characteristics that they all share is that they are monotonic in $s_{i,j}$ and that they enhance the difference between small similarity values and large ones.\\
The last family instead generates binary, un-weighted networks, in which the connection between two genes is either present (1) or absent (0). Obviously, the use of hard thresholds generates simpler networks, for which concepts such as node connectivity are easier to define and have straightforward interpretations, however they are also highly sensitive to the specific threshold used and lose a substantial amount of information, while technically no information is lost when applying soft thresholds.\\


\subsection{Selection of the adjacency function}
The best adjacency function is usually selected from the chosen family using the scale-free topology criterion. Scale-free topology (SFT) is a condition in which the number $P$ of nodes (i.e., genes) with connectivity $k$ is proportional to a (negative) power of said connectivity: $P(k) \sim k^{-\gamma}$.
The emergence of SFT follows directly from the growth of the network (larger networks are more commonly SFT) and is a property that is also thought to characterize the evolution of biological systems \cite{barabasi1999emergence,albert2000topology}. An important mathematical feature of SFT networks is that they exhibit great tolerance towards errors, making them suitable for the analysis of inherently noisy data such as GE values.
To understand how to verify the SFT criterion, first the concept of node connectivity must be introduced. In an un-weighted (i.e., binary) network, the connectivity of the $i$-th node is the number of nodes it is connected to. This can be generalized for a weighted network as follows:
\begin{equation}
    c_i=\sum_j{a_{i,j}}
\end{equation}
A common way to proceed for the evaluation of SFT, is then to calculate $P(k)$ for various values of $k$, fit the function $\log(P(k)) = -\gamma \log(k)$ with free parameter $\gamma$ and calculate the $R^2$ of the fit.\\
It has been empirically observed that, for example for the power functions, a SFT is more easily reached at higher power values. However, since $s_{i,j}<1$, high power values also mean a contraction of the connectivity and thus a compression of the information towards the lower end of the $[0,1]$ interval. This is often undesirable and therefore a common way to choose the power function in such cases is to plot the $R^2$ of the SFT fit against the mean connectivity of the network and find a compromise between a good $R^2$ (above 0.8) and a non-zero connectivity.

\subsection{Definition of a measure of gene dissimilarity}
Now that the network is fully constructed, it is necessary to define a measure of dissimilarity between pairs of genes, and hence the dissimilarity matrix, that can be used to derive gene modules.
This is usually done through the calculation of the topological overlap matrix (TOM) \cite{ravasz2002hierarchical}. The elements $t_{i,j}$ of the TOM describe how similarly connected the nodes $i$ and $j$ are, and can be defined from the adjacency matrix as follows:
\begin{equation}
    t_{i,j} = \frac{\sum_u{a_{i,u} \cdot a_{u,j}} + a_{i,j}  }{ \min{(k_i,k_j)} + 1 - a_{i,j} }
\end{equation}
Where $k_i$ and $k_j$ are the connectivities of node $i$ and $j$ respectively. This formula has an easy interpretation in case of binary networks. Consider as an example two nodes that are connected to all other nodes in the same way: $a_{i,u} = a_{u,j} \ \forall u$. Then, the numerator of $t_{i,j}$ becomes $\min (k_i,k_j)+a_{i,j}$ (remember $a_{i,i}=0$). If also $a_{i,j}=1$ then $t_{i,j}=1$, showing that two nodes that are connected to the same other nodes, and that are connected to each other, have a topological overlap value of 1.\\
Similarly, if two nodes do not share any connection and are not connected to each other $t_{i,j}=1$.\\
The interpretation is more difficult for weighted networks, but it can be shown that $t_{i,j} \in [0,1]$ and increases when the two nodes share many connections.\\
From the TOM values, it is easy to derive a dissimilarity measure as $d_{i,j} = 1 - t_{i,j}$.


\subsection{Identification of network modules}
There are many ways to identify groups of genes that are well connected to each other. The work described in this thesis uses an average linkage clustering algorithm on the dissimilarity matrix as commonly done in many other studies \cite{d2005does,yip2007gene,kerr2008techniques}.
Average linkage clustering is a particular case of hierarchical clustering, that is a process that starts by treating each element (network nodes in the case at hand) as a separate cluster. Then, it repeatedly merges the two clusters that are closest to each other until all elements are in a single cluster. 

From the definition above, it can immediately be seen that hierarchical clustering needs two things to function:
\begin{itemize}
    \item a function that measures distances between two elements $x$ and $y$: $f(x,y)$. This is straightforward in the network case: the dissimilarity matrix $f(x,y) = d_{x,y}$ is used.
    \item a linkage criterion which measures the dissimilarity between two clusters as a function of the pairwise distances of their elements. There are several ways of defining this, as outlined in \cite{murtagh2012algorithms}. The approach adopted in this work is the average linkage, which defines the dissimilarity between two clusters $X$ and $Y$ with cardinality $|X|$ and $|Y|$ as:
    \begin{equation}
        \frac{\sum_{x\in X,y \in Y}{f(x,y)}}{|X||Y|},
    \end{equation}
\end{itemize}

Note that these criteria define the hierarchy of clusters, but if one is interested in extracting network modules, a further decision regarding the level at which the hierarchy is split must be made. In fact, at the top level, all elements of the network belong to a single cluster, while at the bottom level, every element is its own cluster. The researcher must decide at which intermediate level to observe the network, considering cluster number and size. This is a rather arbitrary choice, as no hard criteria exists.

The identified modules are usually represented in subsequent analyses through their eigengenes and/or their hubs as these are are more stable concepts than the module as a whole \cite{langfelder2007eigengene,liu2016weighted}.\\
Eigengenes are linear combinations of the genes of the module, that are more representative of the module than each of its genes. They are the vectors identified with the principal component analysis \cite{ringner2008principal}. Usually only the first eigengene is used, corresponding to the first component, i.e., the one that explains the largest amount of variance of the module.\\
Hubs instead are the genes with the highest intra-modular connectivity, calculated as $c^M_{i}=\sum_{m\in M}{a_{i,m}}$, where $M$ is a module and $m$ is an index running through all the genes in $M$.

\subsection{Evaluating similarity between networks}
\label{subsec:bkg-deltacon}
Throughout the work described in this document, it was necessary to evaluate the similarity between two weighted networks. This is not a simple task, because the two networks may have a different number of connections. There are many ways to compare networks, as outlined in \cite{}, and the description of all of them is out of the scope of this thesis. The one used in this work is the DeltaCON \cite{koutra2013deltacon}.\\
Its idea is based on comparing the matrix $b_{i,j}$ of the pairwise node affinities of both networks. Node affinity is a concept that aims at quantifying the influence that a certain node $i$ has on another node $j$.
The authors of \cite{koutra2013deltacon} propose to calculate it as follows:
\begin{equation}
    \mathbf{S} = (\mathbf{I} + \epsilon^2\mathbf{C} - \epsilon\mathbf{A})^{-1} 
\end{equation}
Where $\mathbf{I}$ is the identity matrix, $\mathbf{C}$ is the diagonal matrix of the connectivity values $c_i$ and $\mathbf{A}$ is the adjacency matrix. The parameter $\epsilon$ is calculated as $1/(1+\max_i(c_i))$.
The idea behind this formula stems from the fact that, ignoring the $\epsilon^2$-weighted term, $\mathbf{S}$ can be written as:
\begin{equation}
    \mathbf{S} \approx (1-\epsilon \mathbf{A})^{-1} \approx 1 + \epsilon \mathbf{A} + \epsilon^2 \mathbf{A}^2 + ...
\end{equation}
Considering that $k$-th powers of $\mathbf{A}$ encode information on the interaction between $k$-neighbors (just as the matrix $\mathbf{A}$ encodes the interaction between first neighbors), it can be said that $\mathbf{S}$ takes into account all the interactions at different levels, by appropriately discounting them with a decreasing weight (remember $\epsilon < 1$). In addition to this, the $\epsilon^2 \mathbf{D}$ term also considers the total connectivity of each node.\\
The DeltaCON measure then contains a measure of the similarity of the two matrices $\mathbf{S}_1$ and $\mathbf{S}_2$ computed for the two networks:
\begin{equation}
    \delta_c =\sqrt{ \sum_{i,j} ( \sqrt{s_{1,i,j}} - \sqrt{s_{2,i,j}} )^2 }
\end{equation}
This measure of distance is known as Matusita distance \cite{matusita1953estimation} and the authors argue that it is better than other more standard distance functions such as euclidean distance because the square root boosts the values of $s_{i,j}$ (because they are smaller than 1) and thus enhances the sensitivity of $\delta_c$ to small differences between $\mathbf{S}_1$ and $\mathbf{S}_2$.



\section{Data visualization methods}\label{sec:bkg_visualization}
In genetics studies, it is often the case that the data that are analyzed or the results that are derived from them have very high dimension and are thus difficult to intuitively visualize. However, it is often the case that one wants to understand how the data are related to each other with respect to certain criteria. For example it may be interesting to see whether the data are grouped into clusters or show a trend with respect to a certain variable.\\
In order to do this, different visualization techniques have been proposed to address the data dimensionality problem. This section provides a description of two of such techniques: multi-dimensional scaling and dendrograms, that have been employed in many genetics studies.

\subsection{Multi-dimensional scaling}
Multi-dimensional scaling (MDS) is a way of reducing data dimensionality on the basis of a matrix $d_{i,j}$ encoding their pair-wise distances through a distance function $\delta$. 
The goal of MDS is to find, for every data point pair $\vec{p_i}$, a set of coordinates $\vec{x_i}$ such that $\delta(\vec{x_i},\vec{x_j})=d_{i,j}=\delta(\vec{p_i},\vec{p_j})$ for every other data point $\vec{p_j}$.\\
Obviously, this is an ill-posed problem because there are less equations than unknowns ($d_{i,j}$ is a scalar while $\vec{x_i}$ is a vector). 
In order to solve it, further conditions must be imposed. Typically, what is done is to define a \textit{stress} function like the one in the equation below and minimize it.
\begin{equation}
    \Omega = \frac{\sum_{i,j}{(\delta(\vec{x_i},\vec{x_j})-d_{i,j})^2}}{\sum_{i,j}{d_{i,j}^2}}
\end{equation}
Various definitions of $\delta$ generate different MDS variations. The most commonly used ones are euclidean distance, standardized euclidean distance (euclidean distance between the Z-scores, so that the results is not influenced by large scale variations between coordinates), mahalanobis distance and the inverse of the spearman correlation.\\
The dimensionality of the vector $\vec{x_i}$ can be chosen at will, with common choices being 2 and 3 so that the vectors can be visualized in a plot.

\subsection{Other}



==> Materials_and_methods/00-summary.tex <==
\chapter*{Summary}
This part describes the materials and methods of the thesis and follows the same macro structure of the background. It is therefore divided into three chapters: neuroimaging, transcriptomic and imaging genetics. 
It contains a description of all the performed analyses and used datasets. All algorithms and methods taken straight from literature have already been described in the background part and will only be briefly mentioned here, while all modifications and original methods will be more thoroughly detailed.

As already described in chapter \ref{chap:contribution}, the analysis follows the general idea outlined in Fig. \ref{}. Therefore, with neuroimaging, rsfMRI data are analyzed to detect brain regions that may be relevant for autism, while transcriptomic is used to identify a set of genes that may characterize autism. Finally, for imaging genetics, the enrichment of the gene set of interest in the selected brain regions is studied, to seek a reciprocal validation of the two analysis methods.

==> Note.tex <==
\subsubsection*{The proposed work}
The work describes in this thesis can be divided into three main parts: the neuroimaging analysis, the transcriptomic analysis and the imaging genetic analysis, linking the results of the first two.
The main points of the neuroimaging analysis are:
\begin{enumerate}
    \item a confounder-resilient neural network is trained to distinguish ASD subjects from TDC subjects based on their rsfMRI. The network is built in a way that it can exploit the temporo-spatial structure of the rsfMRI, using information from the MR video itself and its optical flow.
    \item the spatial pattern (averaging on the temporal dimension) used by the neural network to classify subjects is calculated with the Smoothgrad \cite{smilkov2017smoothgrad} explainability framework, and the brain regions that are most important for classification are extracted.
\end{enumerate}
The transcriptomic analysis is instead articulated as follows:
\begin{enumerate}
    \item a linear mixed model analysis is used to select lists of genes that allow to distinguish ASD subjects from TDC subjects based on their transcriptional profile, and on regional differences in such profiles.
    \item a weighted gene co-expression network analysis (WGCNA) is used to identify gene modules enriched for the lists of genes found in the previous step.
\end{enumerate}
Finally, the imaging genetic analysis consists in the following steps:
\begin{enumerate}
    \item the gene expression of the gene modules found in the transcriptomic analysis is compared across brain regions in another dataset containing TDC subjects.
    \item it is verified whether the gene expression of the modules found has anomalous values in the regions identified with neuroimaging.
\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection*{Structure of the thesis}
The thesis follows a standard structure and is articulated in 6 parts: background, contribution, materials and methods, results, discussion and conclusion.
Most of these parts, with the exception of the contribution and the conclusion, contain three main chapters: neuroimaging, genetics and imaging genetics, so that readers with different background and interests can easily identify the relevant sections.

The background part contains everything that was not produced by the author of this thesis, and describes the theoretical topics and the state-of-the-art results on which this thesis is founded.

The contribution part, in light of what is reported in the background, details the objectives of this thesis and the advancements with respect to the current knowledge that this work intends to bring. Starting from this section, everything described has been exclusively developed by the author.

The materials and methods and the results parts follow, reporting in detail the methodology of the various analyses and the results obtained. These two parts have the same structure, so that each finding can easily be linked to the data and the analysis steps that generated it.

The results are then critically analyzed, linked together and compared with the current state of the art in the discussion, while the conclusion summarizes the main thesis discoveries and presents possible avenues for future works.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Despite the rapid advances in genetics, most clinical research has not considered genetic and individual differences by conducting “genotype-up” research studies. Instead, the studies have been “phenotype-down” research in which a broad, behaviorally defined group of individuals are considered to establish a research sample. In many studies, all individuals with “autism spectrum disorders” are eligible for participation, and neuroimaging, neuropsychological tests, or other modalities are used to examine differences between subjects with ASD and those with typical development. While this has certainly been a feasible approach, phenotypic or genotypic hetereogeneity may have washed out important clues to the pathophysiology of autism, as well as rendering it impossible to find meaningful biomarkers of autism. To address this, researchers are beginning to perform “deep phenotyping” of biological and clinical variables, as well as behavioral manifestations of ASD, in order to identify subgroups of individuals with ASD that have unique and specific biological abnormalities. Finding abnormalities in basic biologic functions such as sleep \cite{buckley2010rapid} and default neural networks \cite{christakou2013disorder} among subgroups of individuals might represent new treatment targets for those individuals. Those novel therapies then could be tested in the larger ASD population for replication and generalization (or not!)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Results/00-summary.tex <==
\chapter*{Summary}
This part describes the results obtained, following the analyses described in the materials and methods part. To ease the understanding, it is once again separated into three main chapters, one for neuroimaging, one for genetics and one for imaging genetics.
The section titles follow the ones in the materials and methods part, to make it easy to identify the description of the analysis that generated the reported results.

==> Structures/Acknowledgements.tex <==
\begin{acknowledgements}
	I thank ...
\end{acknowledgements}
